Arbitrary Style Transfer via Multi-Adaptation Network

Arbitrary style transfer is a significant topic with research value and application prospect. A desired style transfer, given a content image and referenced style painting, would render the content image with the color tone and vivid stroke patterns of the style painting while synchronously maintaining the detailed content structure information. Style transfer approaches would initially learn content and style representations of the content and style references and then generate the stylized images guided by these representations. In this paper, we propose the multi-adaptation network which involves two self-adaptation (SA) modules and one co-adaptation (CA) module: the SA modules adaptively disentangle the content and style representations, i.e., content SA module uses position-wise self-attention to enhance content representation and style SA module uses channel-wise self-attention to enhance style representation; the CA module rearranges the distribution of style representation based on content representation distribution by calculating the local similarity between the disentangled content and style features in a non-local fashion. Moreover, a new disentanglement loss function enables our network to extract main style patterns and exact content structures to adapt to various input images, respectively. Various qualitative and quantitative experiments demonstrate that the proposed multi-adaptation network leads to better results than the state-of-the-art style transfer methods.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/dyy}}]{Yingying Deng}
received the BSc degree in Automation from University of Science and Technology Beijing in 2017. She is currently working toward the PhD degree in National Laboratory of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences. Her research interests include multimedia analysis, computer vision and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Photo_Tang}}]{Fan Tang}
received the BSc degree in Computer Science from North China Electric Power University in 2013. He is currently working toward the PhD degree in National Laboratory of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences. His research interests include computer graphics, computer vision and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Photo_Dong}}]{Weiming Dong}
is a Professor in the Sino-European Lab in Computer Science, Automation and Applied Mathematics (LIAMA) and National Laboratory of Pattern Recognition (NLPR) at Institute of Automation, Chinese Academy of Sciences. He received his BSc and MSc degrees in Computer Science in 2001 and 2004, both from Tsinghua University, China. He received his PhD in Computer Science from the University of Lorraine, France, in 2007. His research interests include image synthesis and image recognition. Weiming Dong is a member of the ACM and IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{sw}}]{Wen Sun}
received the BSc degree in Central South University in 2016 . She is currently in the third year of his master's degree in Institute of Automation, Chinese Academy of Sciences. Her research interests include image understanding and face recognition. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{image/Photo_Huang}}]{Feiyue Huang}
is the director of Social Network Platform Department, Tencent. He received his BSc and PhD degrees in Computer Science in 2001 and 2008, both from Tsinghua University, China. His research interests include image understanding and face recognition.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Photo_Xu}}]{Changsheng Xu}
is a Professor in National Lab of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences and Executive Director of China-Singapore Institute of Digital Media. His research interests include multimedia content analysis/indexing/retrieval, pattern recognition and computer vision. He has hold 30 granted/pending patents and published over 200 refereed research papers in these areas. Dr. Xu is an Associate Editor of IEEE Trans. on Multimedia, ACM Trans. on Multimedia Computing, Communications and Applications and ACM/Springer Multimedia Systems Journal. He received the Best Associate Editor Award of ACM Trans. on Multimedia Computing, Communications and Applications in 2012 and the Best Editorial Member Award of ACM/Springer Multimedia Systems Journal in 2008. He served as Program Chair of ACM Multimedia 2009. He has served as associate editor, guest editor, general chair, program chair, area/track chair, special session organizer, session chair and TPC member for over 20 IEEE and ACM prestigious multimedia journals, conferences and workshops. He is IEEE Fellow, IAPR Fellow and ACM Distinguished Scientist.
\end{IEEEbiography}
